Generalization of waving-plate theory to multiple interacting swimmers

Early research in aerodynamics and biological propulsion was dramatically advanced by the analytical solutions of Theodorsen, von K\'{a}rm\'{a}n, Wu and others. While these classical solutions apply only to isolated swimmers, the flow interactions between multiple swimmers are relevant to many practical applications, including the schooling and flocking of animal collectives. In this work, we derive a class of solutions that describe the hydrodynamic interactions between an arbitrary number of swimmers in a two-dimensional inviscid fluid. Our approach is rooted in multiply-connected complex analysis and exploits several recent results. Specifically, the transcendental (Schottky-Klein) prime function serves as the basic building block to construct the appropriate conformal maps and leading-edge-suction functions, which allows us to solve the modified Schwarz problem that arises. As such, our solutions generalize classical thin aerofoil theory, specifically Wu's waving-plate analysis, to the case of multiple swimmers. For the case of a pair of interacting swimmers, we develop an efficient numerical implementation that allows rapid computations of the forces on each swimmer. We investigate flow-mediated equilibria and find excellent agreement between our new solutions and previously reported experimental results. Our solutions recover and unify disparate results in the literature, thereby opening the door for future studies into the interactions between multiple swimmers.

==> sections/computing-quantities.tex <==
\subsection{Computing physical quantities}
\label{Sec:computePhys}
%
Now we can calculate some physically meaningful results.
Following Wu, we define the pressure difference across the $m$-th plate in the
positive $y$-direction as
%
\begin{align}
	\Delta p^{(m)}(x) &=
	p(x+0^-i,t) - p(x+0^+i,t)
 = \rho \left(\phi(x+0^-i,t) - \phi(x+0^+i,t) \right)
\end{align}
%
We consider time-averaged quantities and denote these with a hat.
The expectation of a quantity $r(z,t)$ is given by
%
\begin{align}
	\hat{r}(z)=
	\frac{1}{T} \int_{0}^T
	r(z,t)\d t,
\end{align}
%
where $T=2 \pi/\omega$ is the period of oscillation.

\subsection{Time-averaged lift}

The lift exerted by a body is given by
%
\begin{align}
	L = \oint_S p \bn \cdot (0,1) \d S,
\end{align}
%
where $\bn$ is the normal unit vector pointing into the wing.
Note that, since this line integral is scalar valued and taken with respect to arc length, 
reversing the direction of integration 
does not change the integral. 
As such, we split the lift integral into parts along the upper and lower side of the wing:
%
\begin{align}
	L = \oint_{S_+} p_+ \bn_+ \cdot (0,1) \d S_+ + 
	\oint_{S_-} p_- \bn_-\cdot (0,1) \d S_-.
\end{align}
%
For the $m$-th wing, this normal vector is given by
%
\begin{align}
	\bn_\pm^{(m)}(x,t) &= \mp \frac{\left(-\partial_x y^{(m)}(x,t),1\right)}
	{\sqrt{1 + (\partial_x y^{(m)}(x,t))^2}}
		       = \mp \frac{\left( -\partial_x h_1^{(m)}(x,t),1 \right)}
		       {\sqrt{1 + (\partial_x h_1^{(m)}(x,t))^2}},
		       % &= \mp \left( -\partial_x h_1^{(m)}(x,t),1 \right)
		       % \left( 1 - \frac{(\partial_x h_1^{(m)}(x,t))^2}{2} \right)\\
		  % &=  \mp \left( -\partial_x h_c^{(m)} (x)\cos(\omega t) + \partial_x h_s^{(m)}(x) \sin(\omega t),1 \right),
\end{align}
%
where the $\pm$ corresponds to the upper or lower side of the wing.
Therefore, we have
%
\begin{align}
	\oint_{S^\pm} p_\pm \bn_\pm \cdot(0,1) \d S_\pm &= \mp
	\int_{\rm l.e.}^{\rm t.e.} p_\pm(x) 
	\frac{1}{\sqrt{1 + (\partial_x h_1^{(m)}(x,t))^2}}
\sqrt{1 + (\partial_x h_1^{(m)}(x,t))^2}
	\d x = 
	\mp\int_{\rm l.e.}^{\rm t.e.} p_\pm(x,t) \d x.
\end{align}
%
Recall that the pressure can be expressed as parts proportional to $\cos$ and $\sin$:
%
\begin{align}
	p(x,t) &= p_c(x) \cos(\omega t) + p_s(x) \sin(\omega t) = p(x) \cos(\omega t - \phi).
\end{align}
As such, that time-averaged pressure at any point is zero, and the time-averaged lift also vanishes.

This seems to be at odds with experimental results and intuition.
We believe that this discrepancy arises because of our linear theory -- if the forcing (wing motion) is a linear combination
of $\cos(\omega t)$ and $\sin(\omega t)$ then the response (pressure) must also be a linear 
combination of $\cos(\omega t)$  and $\sim(\omega t)$.
A nonlinear theory is required to capture non-zero time-averaged lift values.

To actually compute the lift, it is convenient to transform the spatial integral into the circular domain:
%
\begin{align}
	\int_{\textnormal{l.e.}}^{\textnormal{t.e.}}
	\Delta p^{(m)}(z,t) \d z
	= \oint_{C^{(m)}} p^{(m)}(f(\zeta),t) \frac{\d f}{\d \zeta} \d \zeta 
\end{align}
%
Note that the orientation for $C^{(0)}$ will be opposite to that of the other circles.
We know that $p^{(m)}$ is analytic everywhere except at the leading edge 
where it has a simple pole.
However, we also know that $\d f/\d \zeta=0$ at the leading and trailing edges.
As such, the above integrand is analytic in a neighbourhood of the contour
and can therefore be approximated accurately using the trapezoidal rule.
Manipulating the integral further gives
%
\begin{align}
	L=\oint_{C^{(m)}} p^{(m)}(f(\zeta),t) \frac{\d f}{\d \zeta}(\zeta) 
	\d \zeta 
	 =
	 q^{(m)} \i
	 \int_0^{2 \pi} p^{(m)}(f(\delta^{(m)} + q^{(m)} \e^{\i \theta}),t)
	 \frac{\d f}{\d \zeta}(\delta^{(m)} + q^{(m)} \e^{\i \theta}) 
	 \e^{\i \theta}
	 \d \theta 
	 = 
	 \int_0^{2 \pi} s(\e^{\i \theta})
	 \d \theta 
\end{align}
%
Now, the integral $L$ is approximated by
%
\begin{align}
	L \sim L_N = \frac{2 \pi}{N} \sum_{k=1}^N s(z_k)
\end{align}
%
where $z_k$ are the $N$th roots of unity: $z_k = \e^{2 \pi \i k/N}$.
This approximation converges exponentially fast.

\subsection{Thrust}
We'll now compute the time-averaged thrust.
Since the thrust is a nonlinear quantity, its time-averaged value will generally not be zero,
as in the case of time-averaged lift.
The thrust on the $m$th wing (taken to be positive in the negative $x$-directions) is given as
%
\begin{align}
	T^{(m)}(t) &= \int_{l.e.}^{t.e.} 
	\Delta p^{(m)}(z,t) \frac{\partial h^{(m)}}{\partial x}(z,t) \d z + T_B^{(m)}(t)
\end{align}
%
where $T_B^{(m)}(t)=T_c^{(m)} \cos(\omega t) + T_s^{(m)} \sin(\omega t)$ is the leading-edge suction of the $m$-th wing.
The leading-edge suction force is given by
%
\begin{align}
	T_{c,s}^{(m)} = \frac{\pi^2}{U^2} \left(a_{c,s}^{(m)}\right)^2 K^{(m)}_r \left| f^{\prime \prime}(\gamma^{(m)}) \right|
\end{align}
%
where $K^{(m)}_r$ is the residue of $K(\zeta, \gamma^{(m)})$ at $\zeta = \gamma^{(m)}$.

We can, again, compute the remaining integral in the circular domain.
Splitting $\Delta p$ and $h$ into their $\cos$ and $\sin$ components yields
%
\begin{align}
	\Delta p^{(m)}(z,t) \frac{\partial h^{(m)}}{\partial x}(z,t)
	= &\Delta p^{(m)}_c(z)  \frac{\partial h^{(m)}_c}{\partial x}(z)\cos(\omega t)^2\\
+& \left(\Delta p^{(m)}_c(z)  \frac{\partial h^{(m)}_s}{\partial x}(z)
+ \Delta p^{(m)}_s(z)  \frac{\partial h^{(m)}_c}{\partial x}(z)
	\right)
	\cos(\omega t) \sin(\omega t)\\
+& \Delta p^{(m)}_s(z)  \frac{\partial h^{(m)}_s}{\partial x}(z)\sin(\omega t)^2.
\end{align}
%
The cross terms vanish when the temporal average is taken and we are left with
%
\begin{align}
\left<	\Delta p^{(m)}(z,t) \frac{\partial h^{(m)}}{\partial x}(z,t) \right>
= & \frac{\pi}{\omega} \left(\Delta p^{(m)}_c(z)  \frac{\partial h^{(m)}_c}{\partial x}(z)+
\Delta p^{(m)}_s(z)  \frac{\partial h^{(m)}_s}{\partial x}(z) \right).
\end{align}
%
So the time-averaged thrust is given by
%
\begin{align}
	\hat{T}&=
	\frac{\pi}{\omega} \left( \hat{T}_c^{(m)} + \hat{T}_s^{(m)}+ \int_{l.e.}^{t.e}
 \Delta p^{(m)}_c(z)  \frac{\partial h^{(m)}_c}{\partial x}(z)+
\Delta p^{(m)}_s(z)  \frac{\partial h^{(m)}_s}{\partial x}(z) \d z \right).
\end{align}
%
\subsection{Power}
%
Similarly, the power is given by
%
\begin{align}
	P^{(m)}(t) &= - \int_{l.e.}^{t.e.} 
	\Delta p^{(m)} (z,t)
	\frac{\partial h^{(m)}}{\partial t}(z,t) \d z .
\end{align}
%
Noting that
%
\begin{align}
\left<	\Delta p^{(m)}(z,t) \frac{\partial h^{(m)}}{\partial t}(z,t) \right>
= & \pi\left(\Delta p^{(m)}_c(z)  h^{(m)}_s(z)-
\Delta p^{(m)}_s(z)  h^{(m)}_c(z) \right),
\end{align}
%
allows the time-averaged power to be calculated as
%
\begin{align}
	\hat{P} = 
	- \pi\int_{l.e.}^{t.e.} \Delta p^{(m)}_c(z)  h^{(m)}_s(z)-
\Delta p^{(m)}_s(z)  h^{(m)}_c(z) \d z.
\end{align}
%


==> sections/conformal-map.tex <==
\subsection{Conformal map}%
\label{Sec:conformalMap}
%
The problem in the physical domain can be reduced to a circular domain by means of a conformal mapping.
We consider a conformal map between the physical $D_z$ domain and the multiply connected
circular domain described in section \ref{Sec:circ}.
Due to the linearisation of the boundary condition in section \ref{Sec:Modelling}, the wings are represented in the physical domain as horizontal flat slits.
Thus, we seek to map each boundary circle in $D_\zeta$ to a horizontal slit in $D_z$.
% We can use the prime function to generalise the conformal map of Wu \cite{wu1961swimming} to higher connectivities.
% The key feature of Wu's map, which is the Joukowski map, is that it maps a circle to a horizontal slit.
% The multiply connected analogue of this map it to map multiple circles to multiple horizontal slits.
Such mappings are called ``parallel slit maps'', and can be written in terms of the Schottky--Klein prime function
\cite{Crowdy2006}.

The horizontal slit maps can be written as
%
\begin{align}
%	f(\zeta) &= A
%	\left(
%		\frac{\omega_\alpha(\zeta,\beta)}{\omega(\zeta,\beta)}
%		- \frac{1}{\bar{\beta}^2}
%		\frac{\omega_\alpha(\zeta,1/\bar{\beta})}{\omega(\zeta, 1/\bar{\beta})} 
%	\right)
%	+
%B
	f(\zeta) &= A
	\left(
	\frac{1}{\bar{\beta}^2}
		\K(\zeta,1/\bar{\beta})	-\K(\zeta, \beta)
	\right)
	+
	B
	\label{Eq:map}
\end{align}
%
for any $\beta \in D_\zeta$.
The positive real constant $A$ scales the domain, and the complex constant $B$ shifts the domain.

It is worth pointing out that the number of parameters matches the number of constraints in the map.
In the physical domain, there are $3(M+1)$ constraints since
each of the $M+1$ slits has a three constraints: two for position and one for length.
As for the parameters, in the circular domain there are three parameters for each of the excised circles:
two for position and one for radius.
Additionally, $A$ and $B$ contribute $3$ parameters, and $\beta$ contributes $2$ further parameters.
The Riemann mapping theorem states that conformal maps are unique only up to a three-parameter family,
and we use two of these parameters to specify that the image of $\beta$ is $\infty$, 
leaving one remaining parameter.
Finally, the imaginary part of the image of $C_0$ is constrained to be $\Im[B]$ by properties of the
parallel slit map, which means that we lose another parameter.
As such, there seem to be $3M + 3 + 2 - 1 - 1= 3(M+1)$ parameters remaining,
which matches the number of constraints.

Mapping between the slit domain and the annulus permits analytic constructions of the pressure field.
We write the acceleration potential in $D_\zeta$ as $G$ so that $g(z) = G(\zeta(z))$.
By the conformal invariance of Laplace's equation, the acceleration potential inside the annulus is also analytic:
$\nabla^2 G = 0.$

Since $\mathcal{K}(\zeta, \beta)$ contains a simple pole at $\zeta = \beta$, the mapping also has a simple pole there.
Specifically, by \eqref{Eq:Kpole}, the Laurent expansion of the mapping about $\zeta = \beta$ is given by
%
\begin{align}
	f(\zeta) \sim \frac{A}{\zeta - \beta}.
	\label{Eq:fLaurent}
\end{align}
% \begin{align}
% f(\zeta) &=
% A \left(
% 	\frac{1}{\beta} \K(\zeta/\beta) - 
% \frac{1}{\bar{\beta}} \K(\zeta\bar{\beta})
% \right)
% + B
% \label{Eq:map}
% \end{align}
%
% is an example of a doubly connected ``parallel slit mapping'' derived by \cite{Crowdy2006};
% $f$ transplants the boundary circles of the annulus to a pair of horizontal slits.
% The parameters $A$ and $B$ respectively represent a scaling factor and a shift 
% so that the image of $C^{(0)}$ lies in the interval $[-1,1]$.
% Since $\K$ has a simple pole at $1$ \eqref{Eq:kExpansion}, the parameter $\beta$ represents the pre-image of infinity.
% The target physical domain can be obtained by appropriate choices of $q$ and $\beta$.
% An example of a doubly connected slit map is illustrated in figure \ref{Fig:conformal}.

\subsubsection{Edge points}
On each circle a pair of points $\zeta^{(m)}_\pm$ are mapped to the physical endpoints of the corresponding slit $z^{(m)}_-$. %so that $f(\zeta^{(m)}_\pm)= z^{(m)}_\pm$.
Here the subscript $\pm$ corresponds to the preimages of the left and right endpoints respectively.
Apart from a few special cases that we will detail below, the preimages of the endpoints must be
computed numerically, which can be done using a simple Newton iteration.

It is useful to inspect the behaviour of the mapping near the preimages of the end points.
The map has a second-order zero near the preimages of the endpoints:
%
\begin{align}
    f(\zeta) - f(\zeta^{(m)}_\pm) \sim \tilde{b}_{\pm}^{(m)} (\zeta - \zeta_{\pm}^{(m)})^2 ,\qquad \textnormal{as } \zeta \rightarrow 
    \zeta_\pm^{(m)},
    \label{Eq:asymp1}
\end{align}
%
where $\tilde{b}_\pm^{(m)}$ are constants that depend on the parameters of the mapping.
We may parameterise $\zeta$ near $\zeta_\pm^{(m)}$ on the boundary circle $C^{(m)}$ with $\epsilon \ll 1$ as
%
\begin{align}
\zeta(\epsilon) = \delta^{(m)} + q^{(m)} \e^{\i (\vartheta_\pm^{(m)}+ \epsilon)},\qquad
    \zeta_\pm^{(m)} = \delta^{(m)} + q^{(m)} \e^{\i \vartheta_\pm^{(m)}}.
\end{align}
%
The gradient of $f$ with respect to $\epsilon$ is then
%
\begin{align}
\partial_\epsilon f(\zeta)
\sim 2\i \tilde{b}_\pm^{(m)} \left(q^{(m)} \e^{\i \vartheta_\pm^{(m)}}\right)^2 \left( \e^{\i \epsilon} - 1 \right)
\sim  - 2\epsilon \tilde{b}_\pm^{(m)} \left(q^{(m)} \e^{\i \vartheta_\pm^{(m)}}\right)^2.
\label{Eq:fDerivEps}
\end{align}
%
Since the plates are horizontal and thus have constant imaginary part, the gradient of $f(\zeta)$ as
$\zeta$ varies over $C^{(m)}$ must be pure real.
Accordingly, $\tilde{b}_\pm^{(m)} \e^{2\i \vartheta_\pm^{(m)}}$ must be pure real.
It follows that \eqref{Eq:fDerivEps} implies that \eqref{Eq:asymp1} may be alternatively expressed as
%
\begin{align}
    f(\zeta) - f(\zeta_\pm^{(m)}) \sim {b_{\pm}^{(m)}} \e^{-2\i \vartheta_\pm^{(m)}} (\zeta - \zeta_{\pm}^{(m)})^2 ,\qquad \textnormal{as } \zeta \rightarrow 
    \zeta_\pm^{(m)},
     \label{Eq:asymp2}
\end{align}
%
where $b_\pm^{(m)}$ are now pure real constants.


We now look at the simply and doubly connected versions of the map \eqref{Eq:map} in more detail.

\subsubsection{The simply connected map}
%
The parallel slit map \eqref{Eq:map} may be viewed as the multiply
connected analogue of the Joukowski map.
In particular, the Joukowski can be obtained as a special (simply connected) case of a parallel slit map.
Recall that, in the simply connected case, the function $\K$ is given by $\K(\zeta,\alpha)=-1/(\zeta - \alpha)$.
Upon the choices $A = -1/2$ and $B = -1/(2 \bar{\beta})$, the parallel slit map
\eqref{Eq:map} becomes
%
\begin{align}
	f(\zeta) &= \frac{1}{2} \left( \frac{1}{\zeta - \beta} - \frac{\zeta}{\bar{\beta} \zeta - 1} \right).
\end{align}
%
Sending $\beta\rightarrow0$ then yields the classical Joukowski map $f(\zeta) = (\zeta + \zeta^{-1})/2$.
In this case, the preimages of the slits are given 
analytically as $\zeta^{(0)}_\pm = \pm 1$, and the far-field behaviour is 
%
\begin{align}
    f(\zeta) \sim \frac{1}{2 \zeta}.
\end{align}
%
\subsubsection{The doubly connected map}
%
The doubly connected mapping is given by \eqref{Eq:map} where $\K$ is given in
\eqref{Eq:kExpansion}.
A doubly connected mapping is illustrated in figure \ref{Fig:conformal}.

However, in the doubly connected case, closed-form expressions for the preimages of the endpoints are not available except
in special cases.
One such special case is the `inline' configuration where $\beta = \sqrt{q}$ and the boundary circles
are mapped to parallel slits on the real axis.
In this case, the preimages of the edges are given as
%
\begin{align}
	\zeta^{(0)}_\pm = \pm 1, \qquad 
	\zeta^{(1)}_\pm = \pm \sqrt{q}.
\end{align}
%
% Another special case is the `stacked' configuration where $\beta = \i \sqrt{q}$ and the slits are 
% stacked one above the other.
% In this case, the preimages of the edges are given as\footnote{\textcolor{red}{Check signs again}}
% %
% \begin{align}
% 	\zeta^{(0)}_\pm = \mp \i, \qquad 
% 	\zeta^{(1)}_\pm = \mp \i \sqrt{q}.
% \end{align}
% %
Asides from this special case, the roots must generally be found numerically.% using, for example, a Newton solver.

==> sections/mathematical.tex <==
\section{Mathematical background}
Before solving the mathematical model introduced in section \ref{Sec:Modelling}, we must first introduce
 the main mathematical tools.
\input{sections/prime-function}
\input{sections/conformal-map}


==> sections/prime-function.tex <==
\subsection{The canonical circular domain} \label{Sec:circ}
%
We now define a multiply connected circular domain, denoted by $D_\zeta$, which is canonical in the sense that, by an extension of the Riemann mapping theorem for simply connected domains, any given planar multiply connected region is conformally equivalent to such a domain. 
The domain $D_\zeta$ is taken to be the interior of the unit disc with $M$ excised discs so that there are a total of $M+1$ boundary circles; such a domain is shown in Figure \ref{Fig:MCD} for $M=3$. The unit circle is labelled as $C_{0}$ and the circular boundaries of the excised discs as  $\left\{C_{j} | j = 1, \dots , M \right\}$. The excised discs have centers $\left\{\delta_j | j = 1, \dots , M \right\}$ and radii $\left\{q_j | j = 1, \dots , M \right\}$. 
A multiply connected extension of the Riemann mapping theorem guarantees
that a conformal mapping exists from some
$D_\zeta$ to a given multiply connected domain which, here,  will be the exterior of a set of $M+1$ slits parallel to the $x$ axis. The geometry of the slits will determine the parameters
$\left\{\delta_j, q_j | j = 1, \dots , M \right\}$.
%
\begin{figure}
\centering
\begin{tikzpicture}[remember picture]

\myCanCircQuadDetailedThick

\end{tikzpicture}

\caption{A multiply connected circular domain $D_\zeta$ for $M=3$. $C_{0}$ denotes the unit circle and $\left\{C_{j}| j = 1,\cdots, 3\right\}$ denotes the boundaries of the
excised discs with centers $\delta_j$ and radii $q_j$. The grey colour denotes regions that are outside the domain of definition.}

\label{Fig:MCD}
\end{figure}
%
For example, in the simply connected case ($M=0$), the canonical circular domain is the unit disc. 
In the doubly connected case ($M=1$), the canonical circular domain may be taken to be a 
concentric annulus without loss of generality. 
A typical quadruply connected ($M=3$) circular domain is illustrated in figure \ref{Fig:MCD}. 
In general, every point on the circle $C_j$ satisfies
%
\begin{align}
|\zeta -\delta_j|^2 = (\zeta - \delta_j)(\overline{\zeta} - \overline{\delta}_j) = q_j^2. \label{Eq:mob1}
\end{align}
%
Moreover, every circle $C_j$ has an associated M\"obius map defined by
%
\begin{align}
\theta_j(\zeta) = \delta_j + \frac{q_j^2 \zeta}{1 - \overline{\delta}_j \zeta}.
\label{Eq:mobMap}
\end{align}
%
These M\"obius maps have a specific geometrical meaning\footnote{\textcolor{red}{Check that this is the right way round.}}. 
For $j>0$, we define $C_j^\prime$ to be the circle obtained by reflecting the circle $C_j$ in the unit disc $C_0$. 
Using \eqref{Eq:mob1}, it is possible to show that the image of $C_j^\prime$ 
in the M\"obius map $\theta_j$ is simply the circle $C_j$. 
Therefore, each M\"obius map $\theta_j$ represents the reflection of the disc $C_j$ in the unit circle $|\zeta| = 1$. 

\subsection{The prime function associated with $D_\zeta$}
\label{Sec:primeFunction}

%
There is an important function associated with any
circular domain of the kind $D_\zeta$ described above: it is known as the (Schottky-Klein) prime function.


Its many uses for solving applied problems involving multiply connected domains is the topic of a recent monograph by one
of the authors \cite{CrowdyBook} and, in this paper, we will summarize and deploy a number of theoretical results set out in more detail there.

%In the general multiply connected case, the prime function may be expressed as the infinite product
%
%\begin{align}
%\omega(\zeta,\alpha) = (\zeta-\alpha) \prod_{\theta \in %\Theta^{\prime \prime}} \frac{(\zeta - %\theta(\alpha))(\alpha - \theta(\zeta))}{(\zeta - %\theta(\zeta))(\alpha - \theta(\alpha))}. %\label{Eq:skpDef}
%\end{align}
%
%where $\Theta^{\prime \prime}$ is the Schottky group of reflections [\textcolor{red}{COMPLETE}].

The prime function of a given domain $D_\zeta$ will be denoted throughout this paper by
\begin{equation}
    \omega(\zeta,\alpha)
    \end{equation}
    where we view it as a function of two variables, even though it also depends on the parameters
    $\lbrace \delta_j, q_j | j=1, \cdots, M \rbrace$
characterizing the domain $D_\zeta$.    
The prime function satisfies some important functional
relations.

First
it is anti-symmetric in its arguments:
%
\begin{align}
    \omega(\zeta, \alpha) = - \omega(\alpha,\zeta).
    \label{Eq:primeSymmetric}
    \end{align}
%
It also satisfies the functional identity
%
\begin{align}
    \overline{\omega\left(\frac{1}{\overline{\zeta}}, \frac{1}{\overline{\gamma}}\right)} =- \frac{1}{\zeta \gamma} \omega(\zeta, \gamma).
    \label{Eq:prime2}
\end{align}
%
A final identity that will be important here concerns a ratio of prime functions, namely, 
%
\begin{align}
    \frac{\omega(\theta^{(j)}(\zeta),\gamma_1)}
    {\omega(\theta^{(j)}(\zeta), \gamma_2)}
    &= \beta^{(j)}(\gamma_1,\gamma_2)
    \frac{\omega(\zeta,\gamma_1)}
    {\omega(\zeta, \gamma_2)},
        \label{Eq:primeBeta}
\end{align}
%
where
the first argument $\zeta$
has been transformed by one
of the M\"obius maps (\ref{Eq:mobMap}).
Expressions for the function $\beta^{(j)}(\gamma_1,\gamma_2)$, and how to evaluate it, can
be found  in
\cite{CrowdyBook}.

%
%\begin{align}
%\beta_j(\gamma_1,\gamma_2) = \prod_{\theta_k \in %\Theta_j} \frac{(\gamma_1 - \theta_k(B_j))(\gamma_2 - %\theta_k(A_j))}{(\gamma_1 - \theta_k(A_j))(\gamma_2 - %\theta_k(B_j))} \label{Eq:betaDef}
%\end{align}
%
%where $\Theta_j$ denotes all compositions of the basic %mappings of the group $\Theta$ which do not have a %positive or negative power of $\theta_j$ at the %right-hand end.
%$A_j$ and $B_j$ are constants defined in
 %chapter 12 of \cite{Baker1897}.
 
Another important tool in our theory is the auxiliary function $\K(\zeta,\alpha)$ defined by the (parametric) logarithmic derivative
%
\begin{align}
	\K(\zeta, \alpha) = {\partial \over \partial \alpha}
	\log \omega(\zeta,\alpha).
\end{align}
%
%It will be convenient to use
%the notation 
%\begin{align}
%	\K(\zeta, \alpha) = {\omega_2(\zeta,\alpha) \over \omega(\zeta,\alpha)}
%\end{align}
%where 
%$\omega_2(\zeta,\alpha)$ refers to a derivative of the prime function with respect 
%to its second argument.

One important feature of $\K$ is that it possesses a simple pole of residue $-1$ at $\zeta = \alpha$:
%
\begin{align*}
    \K(\zeta, \alpha) \sim -\frac{1}{\zeta - \alpha},\qquad\textnormal{as }\zeta \rightarrow \alpha.
    \label{Eq:Kpole}
\end{align*}
%
Additionally, when viewed geometrically
as a conformal mapping of $D_\zeta$
the function $\K$ has special properties when $\alpha$ lies on one of the boundary circles. 
In this case, $\K$ maps all boundary circles $C^{(m)}$ ( $m=0,\dots, M$) to straight parallel lines at some angle of inclination to the horizontal axis.
This geometrical picture is phrased mathematically in the following lemma, which is proved in appendix \ref{Ap:proof}
%
\begin{lemma} \label{lemma}
If
%
\begin{align}
\alpha = \e^{\i \vartheta} \quad \textnormal{or} \quad    \alpha = \delta^{(j)} + q^{(j)} \textrm{e}^{\i \vartheta} 
\end{align}
%
for some $j = 1, \dots, M$ with $0\leq \vartheta <2 \pi$ then
%
\begin{align}
    \K(\zeta, \alpha) = d^{(m)} + \i \eta \e^{-\i \vartheta}, \qquad
    \zeta \in C^{(m)}
\end{align}
for all $m = 0, \dots, M$, where $d^{(m)}$ are constants and $\eta \in \mathbb{R}$.
\end{lemma}
%


The simply and doubly connected cases, $M=0$ and $M=1$ respectively, are of particular interest since the theory then encapsulates the single plate case considered by Wu and the two-plate case which is important in capturing basic interaction effects between swimming plates. This paper will focus on studying these two cases in detail, it being emphasized, however, that the general theory applies to any number of swimming plates.


\subsubsection*{The simply connected, or ``single plate'', case}
%
In the simply connected case, the prime function is  given by
%
\begin{align}
	\omega(\zeta, \alpha) = \zeta - \alpha.
	\label{sccase}
\end{align}
%
This means that 
%
\begin{align}
	\K(\zeta, \alpha) = -{1 \over \zeta - \alpha}
\end{align}
which is a rational function with a simple pole.

\subsubsection*{The doubly connected, or ``two-plate'',  case}

In the doubly connected, or ``two-plate'', case,
 the
circular preimage domain $D_\zeta$
can be taken to be the annulus $q\leq|\zeta|\leq1$.
The excised circle can always be made to be concentric with $C_0$ on use of the freedoms implicit in the Riemann mapping theorem.
The prime function associated with this domain is
given, up to a multiplicative factor, by
%
\begin{align}
    \omega(\zeta, \alpha) = -\alpha P(\zeta/ \alpha),
\end{align}
%
where we use the same function name $\omega$ and
%
\begin{align}
P(\zeta) &= \left(1- \zeta\right) \prod_{k=1}^{\infty} \left(1 - q^{2k} \zeta \right) \left( 1- q^{2k} \zeta^{-1}\right).
\label{Eq:Pdef}
\end{align}
%
The function
 $P(\zeta)$ is clearly a function of the
 radius $q$, as well as $\zeta$, but this dependence is dropped in our notation
for clarity.
Note that, as $q \to 0$,
\begin{equation}
    \omega(\zeta,\alpha) \to (\zeta-\alpha)
\end{equation}
thereby retrieving the simply connected, or ``single-plate'' , case (\ref{sccase}).
%
%\begin{align}
%	P(\zeta) \sim 1 - \zeta \qquad \qquad \textrm{as } q %\rightarrow 0
%\end{align}
%
%along with other salient properties expounded by %\cite{Baker1897}.
%We shall use this fact to establish the connection between the doubly connected case in this work 
%and the simply connected case of previous works.
% We shall show that every solution can be expressed in terms of the logarithmic derivative of the prime function.
The auxiliary function $\K$ becomes (up to an additive constant)
%\textcolor{red}{Peter, change below}
%
\begin{align}
	\K(\zeta,\alpha) &= -\frac{\zeta}{\alpha^2} \frac{P^\prime(\zeta/\alpha)}{P(\zeta/\alpha)} 
=
 \frac{\zeta}{\zeta - \alpha} + 
	\sum_{k=1}^\infty \frac{\alpha q^{2k}}{\zeta - \alpha q^{2k}} -
		\frac{q^{2k} \zeta}{\alpha - q^{2k} \zeta} .
		\label{Eq:kExpansion}
\end{align}
%
%which can be suitably truncated for computation.

==> sections/solution.tex <==
\section{Solution}
\label{Sec:Solution}

Having introduced all the necessary mathematical objects, we now solve the multiple-swimmer problem introduced in Section \ref{Sec:Modelling}.
%
First, due to the structure of the conformal map \eqref{phimap} near $\zeta^-_{m}$, the acceleration potential $\APot(\zeta,t)$ must possess a simple pole at each $\zeta^-_{m}$ in order to properly capture the square-root singularity in pressure known to exist at the leading edge of each wing. 
\nick{Here too we need to reword because the logic is misstated regarding the pressure singularity.}
\Peter{Change this based on the discussion with Nick.}
As discussed in Section \ref{Sec:Kfun}, the function $\hat{\K}(\zeta, \alpha)$ from \eqref{Eq:hatKdef} possesses a simple pole at $\zeta=\alpha$, allowing us to extract the singularities from $\APot(\zeta,t)$ as follows
\begin{align}
	\APot(\zeta,t) = L(\zeta,t) + \sum_{m=0}^M a_{m}(t) \hat{\K}\left(\zeta,\zeta^-_{m}\right)+c(t). 
	\label{Eq:singularityExt}
\end{align}
where $L(\zeta,t)$ is called the regular part of the solution and is {\em finite} on all boundary components. Due to the rotation $\i\e^{\i \vartheta_k}/\alpha$ introduced in \eqref{Eq:hatKdef}, the coefficients $a_m(t)$ are all real.
\Peter{Some important stuff here was deleted... Like the explanation of why $a_m$ are real.
And I think it's important to explicate the asymptotic behaviour of $F$ and $\hat{\K}$ so that the reader sees that they are almost the same.
}

Importantly, Section \ref{Sec:Kfun} shows that each function $\hat{\K}\left(\zeta,\zeta^-_{m}\right)$ assumes a constant imaginary part on each boundary component. Therefore, evaluating the imaginary part of \eqref{Eq:singularityExt} on the boundary gives
\begin{align}
	 \Im \left[ L(\zeta,t)  \right] 
	 = \Psi_{m}(\zeta,t) + d_{m}(t) , \qquad\qquad \zeta \in C_{m},\,  m = 0,\dots, M
\label{Eq:schwarz3}
\end{align}
where $\Psi_{m}$ is boundary data that is known through \eqref{Eq:PsiDefn}, and the (time-dependent) constants $d_m$ arise from two sources: first, from anti-differentiating \eqref{Eq:convDeriv} to obtain $\Psi_m$, and second from the evaluation of $\hat{\K}\left(\zeta,\zeta^-_{m}\right)$ on each boundary. In our formulation, it is unnecessary to distinguish between these two contributions, and so we lump them together into $d_m$. One of these can be absorbed into $c$, and so, without loss of generality, we take $d_0=0$.

\nick{I hate to be the bearer of bad news, but we use $c$ for chord, so we better pick a different letter for the constant. Maybe just capital $C$? Is that used?}

% MISC NUGGETS THAT MIGHT BE USEFUL
%Since the vertical velocity on the wing is bounded (it is specified by the no-flux condition \ref{Eq:bc}), the imaginary part of $\aPot$ is also bounded by \eqref{Eq:velPres}.

%Physically, $a_{m}(t)$ represent the leading-edge suction coefficients; determining these coefficients is a key part of the problem.

%$c$ is a (time-dependent) constant that enforces the far-field behaviour \eqref{Eq:presFF}}.

Now, \eqref{Eq:schwarz3} takes the form of a modified Schwarz problem as discussed in Section \ref{Sec:Schwarz}. An integral formula for the solution  therefore follows from (\ref{eq:dgc3}):
% \begin{align}
% 	L(\zeta,t) &=	\frac{1}{2 \pi}  \int_{\partial D_\zeta}\left(\Psi_{m}(\zeta^\prime,t) + d_{m}(t) \right)
% 	\left(\d \log \omega(\zeta^\prime,\zeta)
% 	+ \d \log\overline{\omega}\left( \overline{\zeta}^\prime, \frac{1}{\zeta} \right)
% 	\right).
% 	\label{Eq:schwarzSol}
% \end{align}
\begin{align}
	L(\zeta,t) &=	\frac{1}{2 \pi}  \int_{\partial D_\zeta}\left(\Psi_{m}(\zeta^\prime,t) + d_{m}(t) \right)
	\left [{\mathcal K}(\zeta,\zeta') {d \zeta'
\over \zeta'} + \overline{{\mathcal K}}(1/{\zeta},\overline{\zeta'}){d \overline{\zeta'}
\over \overline{\zeta'}} 
\right ] + C,
	\label{Eq:schwarzSol}
\end{align}
where the (time-dependent) constants $d_m$ can be determined by enforcing compatibility conditions.
%Since a modified Schwarz problem assumes the analytic function remains {\em finite} on the boundary, 
The singular coefficients $a_m(t)$ are not determined by this formula and must be treated separately.

\nick{Remember, we need to do that final consistency check on this formula; i.e. In the annulus case, derive the series coefficients using this formula and make sure they agree with what we have been using in the code.}




\subsubsection*{Harmonic motions}
%
The analysis of the previous section follows exactly when the wings are undergoing harmonic motions but $\Psi_m$
is replaced with its vectorised equivalent \eqref{Eq:vectorBC}.
Using the harmonic motion representation from section \ref{Sec:harmonic},
the solution \eqref{Eq:schwarzSol} is expressed as $\bL = [L^c(\zeta)\,\,\,\, L^s(\zeta)]^T$.
Explicit expressions for $\bL$ -- i.e. without integrals -- are available for simple cases such as when all the wings are heaving in-phase.
We derive such expressions in appendix \ref{Ap:exact}.

\input{sections/singular}

% \input{sections/computing-quantities}

